SWAT Watershed Model Calibration using Deep Learning

Watershed models such as the Soil and Water Assessment Tool (SWAT) consist of high-dimensional physical and empirical parameters. These parameters need to be accurately calibrated for models to produce reliable predictions for streamflow, evapotranspiration, snow water equivalent, and nutrient loading. Existing parameter estimation methods are time-consuming, inefficient, and computationally intensive, with reduced accuracy when estimating high-dimensional parameters. In this paper, we present a fast, accurate, and reliable methodology to calibrate the SWAT model (i.e., 21 parameters) using deep learning (DL). We develop DL-enabled inverse models based on convolutional neural networks to ingest streamflow data and estimate the SWAT model parameters. Hyperparameter tuning is performed to identify the optimal neural network architecture and the nine next best candidates. We use ensemble SWAT simulations to train, validate, and test the above DL models. We estimated the actual parameters of the SWAT model using observational data. We test and validate the proposed DL methodology on the American River Watershed, located in the Pacific Northwest-based Yakima River basin. Our results show that the DL models-based calibration is better than traditional parameter estimation methods, such as generalized likelihood uncertainty estimation (GLUE). The behavioral parameter sets estimated by DL have narrower ranges than GLUE and produce values within the sampling range even under high relative observational errors. This narrow range of parameters shows the reliability of the proposed workflow to estimate sensitive parameters accurately even under noise. Due to its fast and reasonably accurate estimations of process parameters, the proposed DL workflow is attractive for calibrating integrated hydrologic models for large spatial-scale applications.

==> Sections/SWAT_DL_Figures.tex <==
%****************************************;
%                                        ;
%  NAME                                  ;
%    SWAT_DL_Figures.tex                 ;
%                                        ;
%  WRITTEN BY                            ;
%    Maruti Kumar Mudunuru               ;
%                                        ;
%****************************************;

%---------------------------------------------------;
%  Figure-1: NHDPLUS-based SWAT for ARW study site  ;
%---------------------------------------------------;
\begin{figure}
  \centering
    \includegraphics[width = 1.05\textwidth]{Figures/Study_Site.png}
  %
  \caption{\textbf{NHDPlus-based SWAT model for ARW:}~This figure shows the watershed delineation and data products used to develop the \texttt{SWAT} model for our study site.
  The top left figures show the delineation of YRB into different watersheds, among which is our ARW study site.
  It also shows the DEM used for modeling ARW and associated stream gauge at the watershed outlet.
  The top right figures show the spatially varying slope and soil data within the study site.
  The bottom left figure shows the delineation of third-order streams in ARW. 
  The bottom right figures show the spatially varying land cover (primarily evergreen) and the number of HRU employed in the \texttt{SWAT} model.
  \label{Fig:SWAT_ARW_Study_Site}}
\end{figure}

%-----------------------------------------------------;
%  Figure-2: SWAT simulations vs. observational data  ;
%-----------------------------------------------------;
\begin{figure}
  \centering
    \includegraphics[width = 0.95\textwidth]{Figures/Mean_vs_Obs_q.pdf}
  %
  \caption{\textbf{SWAT model simulations vs. observational data within calibration period:}~This figure compares the synthetic data generated based on NHDPlus-based \texttt{SWAT} model with observational data for the ARW study site.
  The dark brown color dashed line represents the ensemble mean of 1000 \texttt{SWAT} model simulations.
  The light orange color region represents the standard deviation of ensembles.
  The black-colored line corresponds to the observed streamflow data.
  \label{Fig:SWAT_sim_vs_obsdata}}
\end{figure}

%------------------------------------;
%  Figure-3: Deep learning workflow  ;
%------------------------------------;
\begin{figure}
  \centering
    \includegraphics[width = 0.95\textwidth]{Figures/SWAT_DL_Workflow.pdf}
  %
  \caption{\textbf{Proposed deep learning workflow for the \texttt{SWAT} model calibration:}~A pictorial description of the proposed DL workflow to estimate parameters and calibrate the \texttt{SWAT} model using observational discharge.
  Ensemble simulations generated by the \texttt{SWAT} model are used to train, validate, and test the DL-enabled inverse models.
  The observational data is then provided as an input to the developed DL models to estimate site-specific parameters.
  These parameters are then used by the \texttt{SWAT} model to simulate discharge and compare with the observational data.
  \label{Fig:DL_Workflow_SWAT}}
\end{figure}

%-----------------------------------------------------------;
%  Figure-4: A tuned DL-enabled inverse model architecture  ;
%-----------------------------------------------------------;
\begin{figure}
  \centering
    \includegraphics[width = 0.95\textwidth]{Figures/Tuned_Baseline_Model.pdf}
  %
  \caption{\textbf{A tuned DL-enabled inverse model architecture:}~This figure shows a pictorial description of a deep convolutional neural network to estimate the \texttt{SWAT} model parameters.
  This DL model inversely maps simulated discharge to 21 different conceptual parameters.
  Hyperparameter tuning is performed to arrive at this CNN architecture.
  This DL-enabled inverse model is a multi-task learning model, which accounts for the correlation between different \texttt{SWAT} parameters during training.
  \label{Fig:DL_Baseline_Model}}
\end{figure}

%--------------------------------------------;
%  Figure-5: DL-enabled inverse models loss  ;
%--------------------------------------------;
\begin{figure}
  \centering
    \subfigure[21-parameter model:~Loss]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/Loss_BM_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[7-parameter model:~Loss]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/Loss_7p_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[1-parameter model:~Loss (SFTMP)]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/Loss_1p_lr_1e-5_m4_q_500.png}}
    %
  \caption{\textbf{Loss metrics of best inverse models:}~This figure shows the overall training and validation loss of three different DL-enabled inverse models.
  The overall loss of the 21-parameter model is the sum of the loss of individual \texttt{SWAT} parameters.
  Similarly, the overall loss of the 7-parameter model is the sum of the loss of the top seven sensitive \texttt{SWAT} parameters.
  The loss of the 1-parameter model corresponds to the SFTMP, which is the top sensitive parameter.
  \label{Fig:DL_Models_Loss_SFTMP}}
\end{figure}

%-----------------------------------------------------------;
%  Figure-6: DL-enabled inverse models predictions (SFTMP)  ;
%-----------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[21-parameter model:~Training]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_train_14_BM_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[21-parameter model:~Validation]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_val_14_BM_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[21-parameter model:~Testing]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_test_14_BM_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[7-parameter model:~Training]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_train_14_7p_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[7-parameter model:~Validation]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_val_14_7p_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[7-parameter model:~Testing]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_test_14_7p_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[1-parameter model:~Training]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_train_14_1p_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[1-parameter model:~Validation]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_val_14_1p_lr_1e-5_m4_q_500.png}}
    %
    \subfigure[1-parameter model:~Testing]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/IT_test_14_1p_lr_1e-5_m4_q_500.png}}
  %
  \caption{\textbf{Predictions of DL-enabled inverse models for the SFTMP:}~This figure shows one-to-one plots of best inverse models for the most sensitive parameter, SFTMP (units in $^{\mathrm{o}}\mathrm{C}$).
  It compares the DL estimation with the ground truth for training, validation, and test datasets. 
  Each blue dot represents a realization from the corresponding train/validation/test set of ensembles. 
  The red line is the one-to-one line.
  \label{Fig:DL_Models_SFTMP_Predictions}}
\end{figure}

%--------------------------------------------------------------;
%  Figure-7: Performance of DL-enabled inverse models (SFTMP)  ;
%--------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[1- vs. 21-parameter model]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/b_1p_test_14.png}}
    %
    \subfigure[7- vs. 21-parameter model]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/b_7p_test_14.png}}
    %
    \subfigure[1- vs. 7-parameter model]
    {\includegraphics[width = 0.295\textwidth]{Figures/TrainValTest_Loss_Predictions/7p_1p_test_14.png}}
    %
  \caption{\textbf{Comparison of the best DL-enabled inverse models in predicting SFTMP on test dataset:}~This figure provides a one-to-one plot of percent errors in predicting SFTMP.
  DL analysis is shown for test data, where each data point represents a realization from this set.
  The red line is the one-to-one line.
  DL models (i.e., 1-parameter and 7-parameter models) guided by sensitivity analysis slightly outperform 21-parameter models.
  This is because the percent errors of such models are less than the 21-parameter model.
  \label{Fig:DL_SFTMFP_PercentError_Testdata}}
\end{figure}

%------------------------------------------------------------------;
%  Figure-8: Sensitivity of estimated parameters to noise (SFTMP)  ;
%------------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[Noise added to a test realization]
    {\includegraphics[width = 0.485\textwidth]{Figures/Sensitivity_Noise/SFTMP_boxplot_test.pdf}}
    %
    \subfigure[Noise added to observational discharge (calibration period)]
    {\includegraphics[width = 0.485\textwidth]{Figures/Sensitivity_Noise/SFTMP_boxplot_obs.pdf}}
    %
  \caption{\textbf{Sensitivity of DL estimated parameters to noise (SFTMP):}~This figure shows the sensitivities of the DL-enabled inverse models to different noise levels added to the simulated and observational discharge.
  The results are based on the best models represented by the colors filling the box plots.
  The left figure shows the variation in SFTMP (units in $^{\mathrm{o}}\mathrm{C}$) with noise level for a simulated test realization.
  The markers in the left figure show the synthetic truth and compare with the predictions under no noise.
  Similarly, the markers in the right figure show the mean estimated value from the three best models and compare with the estimations under no noise.
  The estimations of the most sensitive parameter SFTMP are robust to noise.
  The maximum possible variation in SFTMP is less than 0.5$^{\mathrm{o}}\mathrm{C}$ even under 25\% relative observational errors.
  \label{Fig:Params_SenstoNoise}}
\end{figure}

%--------------------------------------------------------;
%  Figure-9: DL vs GLUE estimated parameters (Obs data)  ;
%--------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[KGE vs. SFTMP]
    {\includegraphics[width = 0.475\textwidth]{Figures/Calib_Params_Metrics/0_KGE_vs_SFTMP.pdf}}
    %
    \subfigure[$R^2$-score vs. SFTMP]
    {\includegraphics[width = 0.475\textwidth]{Figures/Calib_Params_Metrics/0_R2_vs_SFTMP.pdf}}
    %
    \subfigure[NSE vs. SFTMP]
    {\includegraphics[width = 0.475\textwidth]{Figures/Calib_Params_Metrics/0_NSE_vs_SFTMP.pdf}}
    %
    \subfigure[logNSE vs. SFTMP]
    {\includegraphics[width = 0.475\textwidth]{Figures/Calib_Params_Metrics/0_logNSE_vs_SFTMP.pdf}}
    %
  \caption{\textbf{Estimated SWAT parameter (SFTMP) using observational data (DL vs. GLUE):}~This figure compares the estimation of SFTMP parameter using observation data with four different performance metrics.
  The calibration sets are identified using the top 10 DL-based inverse models and the GLUE method.
  The blue, red, and light orange colored data points represent the DL estimation, GLUE behavioral set, and ensemble runs parameter space.
  Across the performance metrics, it is evident that estimation using DL-enabled inverse models is well clustered compared to GLUE.
  \label{Fig:DL_vs_GLUE_Obs_Data_Top7Params}}
\end{figure}

%-------------------------------------------------------------;
%  Figure-10: Performance metrics on observational discharge  ;
%             (Calibration and validation periods)            ;
%-------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[Calibration period]{\includegraphics[width = 0.485\textwidth]{Figures/Calib_Params_Metrics/Top_10_R2_NSE_KGE_cnn.pdf}}
    %
    \subfigure[Validation period]{\includegraphics[width = 0.485\textwidth]{Figures/Valid_Metrics/Top_10_R2_NSE_KGE_cnn_ValPeriod.pdf}}
    %
    \subfigure[{\scriptsize Calibration period:~KGE-based best set (KGE = 0.74)}]
    {\includegraphics[width = 0.245\textwidth]{Figures/Calib_Params_Metrics/SWAT_vs_Obs_CNN.pdf}}
    %
    \subfigure[{\scriptsize Validation period:~KGE-based best set (KGE = 0.76)}]
    {\includegraphics[width = 0.245\textwidth]{Figures/Valid_Metrics/SWAT_vs_Obs_ValPeriodCNN.pdf}}
    %
    \subfigure[{\scriptsize Calibration period:~KGE-based best set (KGE = 0.68)}]
    {\includegraphics[width = 0.245\textwidth]{Figures/Calib_Params_Metrics/SWAT_vs_Obs_GLUE.pdf}}
    %
    \subfigure[{\scriptsize Validation period:~KGE-based best set (KGE = 0.75)}]
    {\includegraphics[width = 0.245\textwidth]{Figures/Valid_Metrics/SWAT_vs_Obs_ValPeriodGLUE.pdf}}
    %
    \subfigure[{\scriptsize Size of mean variation of streamflow vs. time period}]
    {\includegraphics[width = 0.385\textwidth]{Figures/Valid_Metrics/Size_MV_cnn_glue.pdf}}
    %
    \subfigure[{\scriptsize Probability that observational data is contained within the prediction bounds estimated by DL or GLUE}]
    {\includegraphics[width = 0.385\textwidth]{Figures/Valid_Metrics/Prob_MV_cnn_glue.pdf}}
    %
  \caption{\textbf{Performance of DL vs. GLUE estimated parameters on observational data:}~This figure compares the performance of the calibrated parameter sets evaluated by DL (i.e., using the 21-parameter inverse model) and GLUE within and beyond the calibration period.
  The top left figures show the performance metrics of the top 10 sets in the calibration and validation period.
  The performance metrics (e.g., NSE, logNSE) focus on the predictive capability of DL- and GLUE-based calibrated \texttt{SWAT} models in both low and high flows scenarios.
  DL outperforms GLUE across all the metrics.
  The central figures provide the one-to-one plots of the calibrated \texttt{SWAT} model when compared to the observational discharge.
  The discharge predictions are based on the best calibrated set from the DL-enable inverse model and GLUE methods.
  The red line is the one-to-one line.
  Data points based on DL estimated set are closer to the red line when compared to the GLUE-based set. 
  The bottom figure shows the size of the mean variation of streamflow.
  It also provides the probability that the observational data is contained within the prediction bounds (i.e., the light blue or red colored region in Fig.~\ref{Fig:DL_vs_GLUE_CalibTimePeriod}) estimated by calibrated \texttt{SWAT} model.
  The uncertainty in GLUE-based calibration sets prediction, and associated probability is higher than DL.
  \label{Fig:DL_vs_GLUE_Performance_Metrics}}
\end{figure}

%--------------------------------------------------------------------------------------;
%  Figure-11: Comparison of DL vs GLUE calibrated SWAT model (Calibration time period)  ;
%--------------------------------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[Calibration period:~Calibrated SWAT model predictions based on DL estimated parameters]
    {\includegraphics[width = 0.985\textwidth]{Figures/Calib_Params_Metrics/CNN_vs_Obs_q.pdf}}
    %
    \subfigure[Calibration period:~Calibrated SWAT model predictions based on GLUE estimated parameters]
    {\includegraphics[width = 0.985\textwidth]{Figures/Calib_Params_Metrics/GLUE_vs_Obs_q.pdf}}
    %
    \subfigure[Validation period:~Calibrated SWAT model predictions based on DL estimated parameters]
    {\includegraphics[width = 0.985\textwidth]{Figures/Valid_Metrics/CNN_vs_Obs_q_ValPeriod.pdf}}
    %
    \subfigure[Validation period:~Calibrated SWAT model predictions based on GLUE estimated parameters]
    {\includegraphics[width = 0.985\textwidth]{Figures/Valid_Metrics/GLUE_vs_Obs_q_ValPeriod.pdf}}
    %
  \caption{\textbf{Comparison of the calibrated \texttt{SWAT} model (DL vs. GLUE) with observation data:}~This figure compares the predictions of the calibrated \texttt{SWAT} model with observational data within and beyond the calibration period.
  The solid black line represents the observational data.
  The dashed colored (blue or red) line represents the predictions based on the best calibrated set using DL (i.e., estimation based on 21-parameter inverse model) or GLUE.
  The light colored region (blue or red) represents the prediction uncertainty. This region is calculated by running the \texttt{SWAT} model using the remaining nine calibration sets obtained using DL or GLUE.
  \label{Fig:DL_vs_GLUE_CalibTimePeriod}}
\end{figure}


